Gravitational waves and kicks from the merger of unequal mass, highly compact boson stars

Boson stars have attracted much attention in recent decades as simple, self-consistent models of compact objects and also as self-gravitating structures formed in some dark-matter scenarios. Direct detection of these hypothetical objects through electromagnetic signatures would be unlikely because their bosonic constituents are not expected to interact significantly with ordinary matter and radiation. However, binary boson stars might form and coalesce emitting a detectable gravitational wave signal which might distinguish them from ordinary compact object binaries containing black holes and neutron stars. We study the merger of two boson stars by numerically evolving the fully relativistic Einstein-Klein-Gordon equations for a complex scalar field with a solitonic potential that generates very compact boson stars. Owing to the steep mass-radius diagram, we can study the dynamics and gravitational radiation from unequal-mass binary boson stars with mass ratios up to $q\approx23$ without the difficulties encountered when evolving binary black holes with large mass ratios. Similar to the previously-studied equal-mass case, our numerical evolutions of the merger produce either a nonspinning boson star or a spinning black hole, depending on the initial masses and on the binary angular momentum. We do not find any evidence of synchronized scalar clouds forming around either the remnant spinning black hole or around the remnant boson stars. Interestingly, in contrast to the equal-mass case, one of the mechanisms to dissipate angular momentum is now asymmetric, and leads to large kick velocities (up to a few $10^4\,{\rm km/s}$) which could produce wandering remnant boson stars. We also compare the gravitational wave signals predicted from boson star binaries with those from black hole binaries, and comment on the detectability of the differences with ground interferometers.

==> Response_referee <==
Dear editor,

We thank the referee for carefully reading the manuscript and for their suggestions to improve it, 
which we have tried to follow as closely as possible. 

Our list of responses/changes can be found below. Note that, we have added in red boldface the changes
made in the article. 

Best regards,
                                 the authors [A]

*******************************************************************************************************
*******************************************************************************************************
*******************************************************************************************************

Dear Editors,

in this manuscript the authors present an extensive study of the
orbital merger of two boson stars, extending a previous work carried
out by some of the same authors; in particular they consider in this
work unequal mass binary systems with mass ratios up to q~23. The
authors focus on the characterization of the remnant of such orbital
mergers, investigating the possibility of producing a spinning boson
star or a black hole with a synchronised scalar cloud. They present a
new interesting dynamical mechanism to dissipate angular momentum and
Noether charge, which could not happen in the equal-mass case, and
which is responsable for high-velocity kicks which can have
consequences in the merger rate for these events. Finally they compare
the gravitational wave signals from boson star binaries with those
produced by black hole binaries in the LIGO/Virgo band, and comment on
the possible detectability of these signals.

The authors discuss largely about the possibility of forming spinning
boson stars, and despite not showing evidence of this formation with
the simulations performed, in Fig.6 they present a tentative
prediction of the region in the parameter space where spinning boson
stars could be produced. One general comment is that among the 5 new
binary systems considered in this work, only 2 cases had enough
initial angular momentum to eventually satisfy the quantization
condition at the time of contact (see fig.4), meaning that their
statistic on the formation of spinning BS counts only these 2
simulations (1 if we consider that the more massive one collapsed to
BH after the merger). The same can be said about the formation of
synchronized clouds around BH. Probably a more extensive study in this
direction is needed, out of the scope of this paper. I think that the
authors should emphasize this fact, for example at the end of the
second paragraph of the conclusions.

This is a very interesting work which extend previous results on the
field and present a very detailed discussion; for this reason I
suggest the publication in Physical Review D after some minor
revision. The authors should address the questions and doubts that can
be found below.

*******************************************************************************************************
*******************************************************************************************************
*******************************************************************************************************

Remarks / Questions:

#####################################################################################################
#####################################################################################################

1) I understand that the authors evaluate R99 as the radius containing
99% of the Noether charge evaluated by means of a volume integral. Do
the authors consider the fact that the final object is displaced from
the origin, and evaluate the volume integral with the coordinates
centered on the mass-center (or Noether-charge center) of the remnant
to have a better evaluation of the radius of the object?

[A] We have taken this fact into account and added a sentence in the text in this version of the paper.

#####################################################################################################
#####################################################################################################

2) How do the authors choose the initial positions of the component
BSs in the binary? I would have taken positions such that the center
of mass of the binary system was at the origin. From a calculation
using the component masses and their distance from the origin (as if
they are point-like objects) I see that this is not how the initial
positions were evaluated. Were they chosen like this for a particular
reason?

[A] We have indeed chosen the initial positions for the COM to be at the origin (this is now clarified in the text). Notice that the COM is defined with respect to the initial, static, not "effective" masses.     We have not been able to put all the digits of the position in the text for aesthetic reasons,     but we have considered them in the simulations. For example, for the case C012C022  
    using the numbers in the table for the run, the COM occurs at:

     
        -8.955373279577367*0.365 + 3.0446267204226327*1.0736 = -4.44089209850063e-16
   


#####################################################################################################
#####################################################################################################

3) The authors address the reader to their previous work (ref[39]) for
the definitions of the ADM and the Komar mass and angular momentum. In
this work under review, the authors speak often about the angular
momentum evaluated numerically in their simulations; they call it
J_{z} in Figure 4 and in the text and from the label of figure 4 I
suppose this is the ADM angular momentum; in some cases they call it J
(for example in the first column of page 12 when they talk about the
BH formed), and I suppose that they are still referring to the ADM
angular momentum.

I suggest that the authors fix the notation and use always J_{z}.
Moreover I would make it clearer that J_{z} is the ADM angular
momentum (if this is the case). For example in page 4 where they say
"ADM and the Komar mass, the angular momentum and the Noether charge,
computed as in ref [39]" I suggest to change it into "the ADM and
Komar mass, the XXX angular momentum J_{z}, and the Noether charge N,
computed as in ref [39]", where XXX is either Komar or ADM depending
on what the authors used.

[A] We have modified this following referee's suggestion. The definition of ADM was added as well. 

#####################################################################################################
#####################################################################################################

4) In this respect, at the end of page 12 they talk about the blob of
scalar field passing across the surface at which the ADM mass and
angular momentum are computed. It would be good to specify the radius
of this surface. Moreover, I wonder why the ADM quantities are
evaluated at a surface which is not the outer boundary of the grid. Is
it to have better resolution, or to avoid outer boundary effects?

[A] On page 5 we have specified the extraction radius, we have considered two extraction radii 
    in this paper, i.e, Rext = 100 and Rext = 200. 
    In fact, the feature of the blob passing across the surface is observed on both surfaces. 
    It is just needed to shift and rescale the time properly with the initial mass, contact time and extraction radius. 
    The referee is correct.  We have chosen to evaluate these quantities at those extraction radii because we are located
    in the wave zone but far from the outer boundary condition, where we have enough resolution to calculated them 
    and avoid being spoiled by boundary conditions effects.

#####################################################################################################
#####################################################################################################

5) When they discuss figure 6, I understand how they extrapolate the
area where possible RBS can be formed. In theory though, if you can
form a RBS you are not limited by Mmax of the static configurations,
because Mmax for the rotating configurations can be larger (for
example for mini-boson stars Mmax = 0.663 for the static
configurations, and Mmax=1.315 for the m=1 spinning BS). As a
consequence you could form a RBS with a total mass of the remnant
M1+M2 which is higher than Mmax of the static configurations, without
collapsing to a BH. I think the authors should comment on this in the
text when they describe figure 6.

[A] We thank the referee for pointing out this issue. We have added a comment in light of the referee's point.

#####################################################################################################
#####################################################################################################

6) Page 16: how do they evaluate the factor sqrt(3)? If it comes from
some reference, please provide the reference, if it's your own
calculation maybe you should at least sketch it. Or does sqrt(3) just
come from the assumption that if the 3 detectors had same SNR, the
total SNR is evaluated with the sum of squares
sqrt(SNR1^2+SNR2^2+SNR3^2)? If so it seems to me a very rough
estimate, probably it's better to say "roughly" instead of
"approximately".

[A] We have changed the word "approximately" with the word "roughly" as the referee  
    suggested as we are using the estimate that the referee described  
    as an upper bound (see also the sentence beginning with "As a rough rule of thumb..." in Section IV C ).

#####################################################################################################
#####################################################################################################

(7) Regarding the comment that the referee make in the report, namely:
    "One general comment is that among the 5 new binary systems considered in this work, only 2 cases 
     had enough initial angular momentum to eventually satisfy the quantization condition at the time 
     of contact (see fig.4), meaning that their statistic on the formation of spinning BS counts only
     these 2 simulations (1 if we consider that the more massive one collapsed to BH after the merger). 
     The same can be said about the formation of synchronized clouds around BH. Probably a more 
     extensive study in this direction is needed, out of the scope of this paper. I think that the
     authors should emphasize this fact, for example at the end of the second paragraph of the conclusions."

[A]  We have added a comment in light of the referee's point.

#####################################################################################################
#####################################################################################################

*******************************************************************************************************
*******************************************************************************************************
*******************************************************************************************************
Typos / comments:

#####################################################################################################
#####################################################################################################
a) In equation (10), I am wondering if the authors meant to write in
the LHS $r\times \Psi_{4}$ of if they just meant $\Psi_{4}$. I don't
think there is anything wrong with it, but I think it's more common to
write the multipole expansion of $\Psi_{4}$ and not of $r\Psi_{4}$;
was it a typo?

[A] It is not a typo, it is only a matter of notation. We use that notation ($r\times \Psi_{4}$) for two reasons: 
    (i) the coefficients \Psi^{l,m} are extracted and calculated in spherical surfaces at different extraction radii
     and (ii) to be consistent with notation in the paper I.  

     We have added a comment in light of the referee's point in order to be clearer.
    

#####################################################################################################
#####################################################################################################

b) I noticed that t_{c} was defined in the caption of Table II. I
would repeat in the label of figures 2/3 what t_{c} is to make it
easier to follow/read.

[A] We have added a comment in light of the referee's point.

#####################################################################################################
#####################################################################################################

c) The definition of the Noether current in eq.4 can be confused with
the symbol $J_{z}$ used for the angular momentum. I suggest they
change it from $J^{a}$ to $j^{a}$ to avoid confusion.

[A] We have changed it.

#####################################################################################################
#####################################################################################################
d) Typo in page 11, "the" is repeated twice.

[A] We have fixed it, thanks.

#####################################################################################################
#####################################################################################################
e) At the beginning of page 20 in the conclusions the authors cite
reference [79] regarding stable solitonic BSs. This should be a typo
and they should be citing [78] (Siemonsen and East paper).

[A] We have fixed it, thanks.

*******************************************************************************************************
*******************************************************************************************************
*******************************************************************************************************

